Warped Dynamic Linear Models for Time Series of Counts

Dynamic Linear Models (DLMs) are commonly employed for time series analysis due to their versatile structure, simple recursive updating, ability to handle missing data, and probabilistic forecasting. However, the options for count time series are limited: Gaussian DLMs require continuous data, while Poisson-based alternatives often lack sufficient modeling flexibility. We introduce a novel semiparametric methodology for count time series by warping a Gaussian DLM. The warping function has two components: a (nonparametric) transformation operator that provides distributional flexibility and a rounding operator that ensures the correct support for the discrete data-generating process. We develop conjugate inference for the warped DLM, which enables analytic and recursive updates for the state space filtering and smoothing distributions. We leverage these results to produce customized and efficient algorithms for inference and forecasting, including Monte Carlo simulation for offline analysis and an optimal particle filter for online inference. This framework unifies and extends a variety of discrete time series models and is valid for natural counts, rounded values, and multivariate observations. Simulation studies illustrate the excellent forecasting capabilities of the warped DLM. The proposed approach is applied to a multivariate time series of daily overdose counts and demonstrates both modeling and computational successes.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> old/random.tex <==
When the counts are large and take values in a wide range, then the data is well approximated by a continuous process, and these time series structures can thus be dealt with via classical models. However, when we observe time series where the counts are low and the degree of ``discreteness'' grows, the applicability of continuous models diminishes.  These low count time series are becoming more and more common as data is recorded and analyzed on a smaller and smaller timescale. 

The moment generating function (MGF) of $[\bm \theta | \bm z \in \mathcal{C}]$ is also available:
\begin{equation}
    \label{mgf-slct-n}
    M_{[\bm \theta | \bm z \in \mathcal{C}]}(\bm s) = \exp\left(\bm s' \bm \mu_\theta + \frac{1}{2}\bm s' \bm\Sigma_\theta\bm s\right) \frac{\bar\Phi_n(\mathcal{C}; \bm\Sigma_{z\theta}\bm s + \bm \mu_z, \bm \Sigma_z)}{\bar\Phi_n(\mathcal{C}; \bm \mu_z, \bm \Sigma_z)}.
\end{equation}


\subsection{The STAR Linear Model}
\label{subsec:STAR-lin}
The STAR framework is defined in full generality, but in order to develop more useful theory we must make further distributional assumptions, e.g. the case where $\bm z$ and $\theta$ are both normal.  This results in the STAR linear model:
\begin{equation}
    \label{lm}
    \bm z = \bm X \bm \theta + \bm \epsilon, \quad \bm \epsilon \sim N_n(\bm 0, \bm \Sigma_\epsilon)
\end{equation}
with a Gaussian prior $\bm \theta \sim N(\bm \mu_\theta, \bm \Sigma_\theta)$. Under these modeling assumptions, we can directly apply the selection normal properties and conclude the following:

\begin{theorem}
    \label{star-lm}
    Under \eqref{lm}, the posterior distribution is $[\bm \theta | \bm y] \sim \mbox{SLCT-N}_{n, p}(\bm \mu_z = \bm X \bm \mu_\theta, \bm \mu_\theta, \bm \Sigma_z = \bm X \bm \Sigma_\theta \bm X' + \bm \Sigma_\epsilon, \bm \Sigma_\theta, \bm \Sigma_{z\theta} = \bm X \bm \Sigma_\theta,  \mathcal{C} = g(\mathcal{A}_{\bm y}))$. 
\end{theorem}

The expressions in \eqref{post-mean} and \eqref{post-var} allow computations of the posterior mean and variance, respectively, of the regression coefficients $\bm \theta$. The inverse covariance (or precision) matrix for $\bm z$ simplifies:
$$
\bm \Sigma_z^{-1} = \bm \Sigma_\epsilon^{-1} - \bm \Sigma_\epsilon^{-1} \bm X \left(\bm \Sigma_\theta^{-1} + \bm X'\bm\Sigma_\epsilon^{-1} \bm X\right)^{-1}\bm X' \bm \Sigma_\epsilon
$$
and, when $\bm \Sigma_\epsilon = \sigma_\epsilon^2 \bm I_n$, 
$$
\bm \Sigma_z^{-1} = \sigma_\epsilon^{-2}  \{\bm I_n-  \bm X \left(\sigma_\epsilon^2\bm \Sigma_\theta^{-1} + \bm X'\bm X\right)^{-1}\bm X'\}
$$
which only requires a $p$-dimensional inverse. 

The Gaussian prior in Theorem~\ref{star-lm} is conjugate: Gaussian distributions may be expressed as $[\bm \theta] \sim \mbox{SLCT-N}_{1, p}(\mu_z = 0, \bm \mu_\theta, \Sigma_z = 1, \bm \Sigma_\theta, \bm \Sigma_{z\theta} = \bm 0_p',  \mathcal{C} = \mathbb{R})$. The moments and constraints on $\bm z$ are irrelevant as long as $\bm \Sigma_{z\theta} = \bm 0$. However, the conjugacy suggests a more general prior for $\bm \theta$, namely, the SLCT-N distribution:
\begin{lemma}
\label{lem:conjugacy}
    Consider the prior $\bm \theta \sim \mbox{SLCT-N}_{n_0, p}(\bm \mu_{z_0}, \bm \mu_\theta, \bm \Sigma_{z_0}, \bm \Sigma_\theta, \bm \Sigma_{z_0\theta},  \mathcal{C}_0)$ with the likelihood given by the STAR linear model in \eqref{lm}. The posterior is 
    \begin{align*}
        [\bm \theta | \bm y] \sim \mbox{SLCT-N}_{n_0 + n, p}\Big\{
        &\bm \mu_{z_1} = \begin{pmatrix} \bm \mu_{z_0} \\ \bm X \bm \mu_\theta \end{pmatrix}, 
        \bm \mu_\theta, 
        \bm \Sigma_{z_1} = \begin{pmatrix} \bm \Sigma_{z_0} & \bm \Sigma_{z_0\theta} \bm X' \\ \bm X \bm \Sigma_{z_0\theta}' & \bm X \bm \Sigma_\theta \bm X' + \bm \Sigma_\epsilon \end{pmatrix},  
        \bm \Sigma_\theta, \\
        & \bm \Sigma_{z_1\theta} = \begin{pmatrix} \bm \Sigma_{z_0\theta} \\ \bm X \bm \Sigma_\theta \end{pmatrix},  
        \mathcal{C}_1 = \mathcal{C}_0 \times g(\mathcal{A}_{\bm y}) \Big\}.
    \end{align*}
\end{lemma}

Thus the selection normal distribution is conjugate with the STAR likelihood.  Moreover, we can also show that the selection normal is closed under linear transformations.

\begin{lemma}
\label{lem:linearity}
    Suppose $\bm \theta \sim \mbox{SLCT-N}_{n, p}(\bm \mu_z, \bm \mu_\theta, \bm \Sigma_z, \bm \Sigma_\theta, \bm \Sigma_{z\theta},  \mathcal{C})$ and let $\bm \theta^* \stackrel{d}{=} \bm A \bm\theta + \bm a$ where $\bm A$ is a fixed $q \times p$ matrix and $\bm a \sim N_q(\bm \mu_a, \bm \Sigma_a)$ is independent of $\bm \theta$. 
    
    Then $\bm \theta^* \sim \mbox{SLCT-N}_{n, q}(\bm \mu_z, \bm \mu_{\theta^*}, \bm \Sigma_z, \bm \Sigma_{\theta^*}, \bm \Sigma_{z\theta^*},  \mathcal{C})$ where $\bm \mu_{\theta^*} =\bm A\bm \mu_\theta + \bm \mu_a$, $\bm \Sigma_{\theta^*}= \bm A \bm \Sigma_\theta \bm A' +\bm \Sigma_a$, and $\bm \Sigma_{z\theta^*} = \bm \Sigma_{z\theta} \bm A'$.
\end{lemma}


These particular lemmas give us further insight into how the selection normal and STAR framework are related.  They will also be key building blocks in building the theory of STAR models with time series data, a topic which we take up in the following section.


Furthermore, we can look at transition probabilities of the form $\mathbb{P}(y_t = 0 | y_{t-1} = 0)$.

\begin{equation}
\mathbb{P}(y_t = 0 | y_{t-1} = 0) = \frac{\mathbb{P}(y_t = 0, y_{t-1} = 0)}{\mathbb{P}(y_{t-1} = 0)} = \frac{\int_{-\infty}^0 \int_{-\infty}^0 p(z_t, z_{t-1}) \,d z_t \, d z_{t-1} }{\int_{-\infty}^0 p(z_{t-1}) \,d z_{t-1}}
\end{equation}
where $p(z_t, z_{t-1})$ and $p(z_{t-1})$ are Gaussian with parameters obtained by taking the appropriate subsets of the full joint $\bm \mu_{z_{t|t}}$ and $ \bm \Sigma_{z_{t|t}}$.

More formally, it is the set of points, denoted $R(c_\alpha)$, where $p(\bm y_{t+h} | \bm y_{1:t}) \geq c_\alpha $, where $c_\alpha$ is the largest constant such that $\mathbb{P}(\bm y_{t+h} | \bm y_{1:t}) \in R(c_\alpha)) \geq 1-\alpha$.  This is a definition which can be applied to both continuous and discrete densities, and produces regions which are coherent for the respective data type.  In addition to being coherent, 










Modeling integer-valued time series has been a topic of research for decades, although no single framework has emerged as the clear best choice. Furthermore, examples of such time series have proliferated in recent years, prompting interest in and need for more flexible models capable of handling the many complexities exhibited by this data type. Initial models often sought to replicate the success of ARMA processes by finding analogues suitable for count data. Thinning operators offer one approach to incorporate autoregressive structure for count processes.  Hence these models are often known as discrete AR or integer AR \citep{McKenzieDARMA1986,Alzaid_Al-Osh_1993}.  Since the initial models were introduced, a huge variety of variations and extensions have been proposed, but no single one has dominated. 

Generalized state space models provide another successful paradigm for time series analysis of integer-valued data.  These types of models have traditionally been categorized into two areas, stemming from \cite{Cox1981}: parameter-driven and observation-driven.  In observation-driven models, the state process is treated as an explicit function of past data values.  One example is the Autoregressive Conditionally Poisson (ACP) model framework \citep{Heinen_2003}, which is akin to the integer GARCH (INGARCH), introduced in \cite{Fokianos_Rahbek_Tjostheim_2009}, where a GARCH process is placed on the time-varying rate parameter of a Poisson data model.

Instead of assigning a particular count distribution (or family of distributions) for the data likelihood, we induce a likelihood by \textit{warping} a continuous model, in particular a Dynamic Linear Model (DLM; \citealp{WestHarrisonDLM}). Crucially, this strategy leverages the great modeling power and flexibility  of (continuous) DLMs, yet is coherent for count data. The warping function has two components: a transformation operator that admits distributional flexibility and a rounding operator that ensures a valid data generating process for integer-valued data with coherent forecasts. Transformation to latent Gaussianity has proven to be a successful modeling strategy for count time series \citep{latentgaussiancount_2021}, and promising results have similarly been shown for rounding of continuous data models \citep{RINAR_Kachour_Yao}. Yet these two approaches have not been considered in tandem within the existing time series literature.

Computational tools for performing inference on DLMs have been developed in many major languages.  In R \citep{rlanguage}, for example, one can use \verb|dlm| \citep{petrisDLMPackage} or \verb|KFAS| \citep{HelskeKFAS}.  Python users can employ \hyperlink{https://pydlm.github.io/}{PyDLM} or \hyperlink{https://pypi.org/project/pybats/}{PyBATS}.

DGLMs have proved to be powerful and useful models in many applications, but their reliance on exponential family distributions means they can be limited in scope.  Furthermore, the need for approximation of the posterior puts an exact and fully Bayesian analysis out of reach. In the following section, we present a new way to use DLMs in the analysis of time series of counts, one which has intriguing theoretical backing and promising results in applications.

The warpDLM intuitively combines two longstanding methods/techniques of time series analysis (DLMs and transformations) in a way that makes sense for count data, both naturally discrete and rounded data.  The coupling of rounding and transformation within the warping operation allows us to model a variety of marginal distributions and data features such as zero-inflation and boundedness.  Critically, the warpDLM performs well when multiple of these complexities are present at once, which is where existing models break down.  Furthermore, the warpDLM model framework is defined for multivariate time series, another area where many current approaches fall short. Finally, as we show in the following section, we can actually derive analytic filtering and smoothing distributions for the warpDLM which are not available for many models of time series of counts.



The data-generating process of the warpDLM is defined by the coupling of the likelihood \eqref{likelihood-time} with the continuous-data model $p(\bm z | \bm \theta)$ and the prior $p(\bm \theta)$. The posterior distribution is 

the default approach here is to put Gamma priors on all precisions, the so-called d-inverse-gamma model.

Forecasting is perhaps one of the most important goals in time series analysis. Proper uncertainty quantification about that forecast is also a necessity, so that risk can be considered in the decision making process.  This is one reason why Bayesian methods are so appealing--the end result is the entire distribution. 

Since we are working with Bayesian methods, our forecasts are probabilistic, and thus should not be evaluated using only point error metrics, but also with tools designed to capture how well the forecasts model uncertainty.  One common way to do this is the use of proper scoring rules \citep{czado2009predictive,Gneiting2014probabilisticforecastingreview}.  We calculate seven scoring rules, in line with what is implemented in the \verb|tscount| package.   We have followed the formulas from \cite{tscountR} with the exception of the normalized squared error score, which was modified so that the the distance between the score and 1 is reported.  In this way, low scores implies a better model for all of these rules.

Having settled on which scoring rules to use, there are still many ways to calculate performance across time periods or across series.  We chose to calculate the scores for each forecast, from all series and time points, and count the number of times each method `won'.  The results are reported in Table \ref{tbl:altogetherwin}.

\begin{table}[!hbtp]
\caption{Numbers of time points where each method had the lowest forecasting score. For each scoring rule, the most wins are bolded.}
\begin{center}
\begin{small}
\color{black}
\begin{tabular}{|c |c |c|c|c|c|c|c|}
\hline
&\textbf{sqrt}&\textbf{id}&\textbf{log}&\textbf{pois}&\textbf{nb}&\textbf{np}&\textbf{DGLM}\\ 
\hline
logarithmic&108&\textbf{441}&368& 48& 40&150&345\\ 
\hline
quadratic& 87&\textbf{501}&324& 49& 34&134&371\\ 
\hline
spherical& 73&\textbf{556}&302& 43& 34&139&353\\ 
\hline
rankprob &123&279&347& 73& 71&125&\textbf{482}\\ 
\hline
dawseb&117&328&332&100&119&132&\textbf{372}\\ 
\hline
normsq& 90&212&246& 86&100&131&\textbf{635}\\ 
\hline
sqerror&110&255&389& 63& 68&126&\textbf{489}\\ 
\hline
\end{tabular}
\end{small}
\end{center}
\label{tbl:altogetherwin}
\end{table}

Three of the models stand out: the warped DLM with identity transformation, the warped DLM with log transformation, and the Poisson DGLM.  The nonparametric CDF-based transformation also shows some promise.  

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth,height=\textheight,keepaspectratio]{INGARCH_simulated_series.png}
    \caption{10 simulated series from the forecasting analysis--counts are low and zeroes are prevalent.}
    \label{fig:ingarchsim}
\end{figure}

We can not show all such plots, so we showcase the results for one of the series. For this series, we plot the randomized PIT values against uniform quantiles in Figure \ref{fig:rPIT}.  For a calibrated forecast, we would expect this resulting line to closely follow the 45-degree line. Since we only have 50 forecasts, to show the inherent variability, we have also plotted the sorted values of 100 draws of n=50 values from the uniform distribution.


Looking at the general area of modeling time series of counts, there is also need for in-depth comparisons amongst different methods, particularly in terms of forecasting performance. Amongst Bayesian methods, new developments in approximate time series cross-validation \citep{LFO-CV} might help such analyses. Regardless, the field would greatly benefit from such comparative studies. 

, which can be summarized using any number of posterior summaries.  For example, city officials might be interested in the probability that there will be a high number of calls the next day, in order to better inform staffing and supplies.  Using our results from the particle filter, we can look at the probability that the next-day counts will be greater than the median level of calls from 2018 and 2019.  The results are shown in \ref{fig:particleprobs}.

\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth,height=\textheight,keepaspectratio]{particleprobs.png}
    \caption{The forecasted probability that the next day will have more counts than the median level from 2018-2019.}
    \label{fig:particleprobs}
\end{figure}

Several observations can be gleaned from this chart.  For non-heroin OD calls, the probability of calls over the median level stays consistently high, suggesting that 2021 as a whole has more of these calls.  However, this time series is also very low-count, so the median is also hovering around 1 or 2, which means a small increase may not make a big deal in terms of resource allocation.  The heroin calls show more interesting dynamics, and there is a clear peak in June where greater calls should be expected.  The time series follows a generally seasonal pattern, with lower counts in the winter months and higher counts in the summer months, but there are some clear deviations, such as a relative decrease in July and a spike in November.  Future analyses of this data might look at increasing the forecast horizons (e.g. week-ahead).  If sufficiently accurate, these forecasts would be of great interest to city EMS and fire department planners, and could help save lives.

 Furthermore, given the warped DLM model components, we can directly compute the parameters of the joint smoothing distribution (and thus draw from it), without having to iterate step-by-step. 
 
 
 Another possible calibration diagnostic, as well as a measure of uncertainty quantification, is that of Highest Density Regions, or HDRs \citep{Hyndman_1996, Mukhopadhyay_Sathish_2018}, which is the smallest set of points whose mass sums to some threshold (e.g. 90\%). In addition to being coherent for count data, HDRs have the added benefit of capturing multimodality, which is a feature often seen in count data. For example, there might be a spike at zero, but also another mode closest to the previously observed data point. Unlike quantile-based regions, the HDR need not be a contiguous sequence.
 
 The Gibbs sampling algorithm was used for posterior inference, and a Uniform$(0,10^4)$ prior was placed on the standard deviations; the variances $\bm V$ and $\bm W$ are thus assumed to be unknown and sampled alongside the states. The initial state $\theta_0$ was given a $N(0,3)$ prior.
 
 \begin{comment}
\begin{proof}[Proof (Lemma 3)]
We have from DLM properties (\citesupp{WestHarrisonDLM} Ch 16) that
\begin{equation*}
\begin{pmatrix} z_1 \\ \theta_1 \end{pmatrix} 
\sim N \left[
\begin{pmatrix} F_1a_1 \\ a_1 \end{pmatrix},
\begin{pmatrix} F_1 R_1 F_1' + V_1 & F_1 R_1\\ (F_1 R_1)' & R_1 \end{pmatrix}
\right]
\end{equation*}  Recognizing that
\[
(\bm \theta_1|y_1) = (\bm \theta_1|z_1 \in g(A_{y_1}))
\]
and leveraging the result from \citesupp{ArellanoValle2006}, we have our conclusion.
\end{proof}
\end{comment}
